The Numerical Assembly Technique for arbitrary planar systems based on an alternative homogeneous solution

The Numerical Assembly Technique is extended to investigate arbitrary planar frame structures with the focus on the computation of natural frequencies. This allows us to obtain highly accurate results without resorting to spatial discretization. To this end, we systematically introduce a frame structure as a set of nodes, beams, bearings, springs, and external loads and formulate the corresponding boundary and interface conditions. As the underlying homogeneous solution of the governing equations, we use a novel approach recently presented in the literature. This greatly improves the numerical stability and allows the stable computation of very high natural frequencies accurately. We show this numerically at two frame structures by investigation of the condition number of the system matrix and also by the use of variable precision arithmetic.

==> 05_Uploads/twoBeamFrameEB/myfile.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5.724in,
height=2.504in,
at={(0.96in,0.338in)},
scale only axis,
xmin=0,
xmax=12,
ymin=-60,
ymax=30,
axis background/.style={fill=white},
grid=both,
ylabel style={font=\color{white!15!black}},
ylabel={\Large$\log |f|$},
xlabel style={font=\color{white!15!black}},
xlabel={\Large$\omega$}
]
\addplot [color=mycolor1, forget plot]
  table[row sep=crcr]{%
0.001	-52.346332150166\\
0.12220202020202	-13.9033983196101\\
0.24340404040404	-8.39836959998323\\
0.364606060606061	-5.1778891713784\\
0.485808080808081	-2.89921044679718\\
0.607010101010101	-1.13978258935218\\
0.728212121212121	0.288867456072323\\
0.849414141414142	1.48726920932393\\
0.970616161616162	2.51533786398436\\
1.09181818181818	3.41158552627799\\
1.2130202020202	4.20214110635042\\
1.33422222222222	4.90544133976189\\
1.45542424242424	5.5348600783717\\
1.57662626262626	6.10026426940495\\
1.69782828282828	6.60896720689061\\
1.8190303030303	7.06631685046078\\
1.94023232323232	7.47604132295957\\
2.06143434343434	7.8404077326623\\
2.18263636363636	8.16020168820263\\
2.30383838383838	8.43447920422115\\
2.4250404040404	8.65994388026911\\
2.54624242424242	8.82956747817358\\
2.66744444444444	8.92938776962182\\
2.78864646464646	8.92993632926733\\
2.90984848484848	8.75633999199958\\
3.0310505050505	8.10298131478283\\
3.15225252525252	7.76384829739516\\
3.27345454545455	9.35027482584224\\
3.39465656565657	10.1294664247413\\
3.51585858585859	10.6907802381604\\
3.63706060606061	11.1393979005032\\
3.75826262626263	11.5129226741811\\
3.87946464646465	11.8279587011624\\
4.00066666666667	12.0916823821288\\
4.12186868686869	12.3053633485166\\
4.24307070707071	12.464745049567\\
4.36427272727273	12.5577144789785\\
4.48547474747475	12.5562889000401\\
4.60667676767677	12.3875247729872\\
4.72787878787879	11.7540217452907\\
4.84908080808081	11.3717804436034\\
4.97028282828283	13.0077889278114\\
5.09148484848485	13.8210342178004\\
5.21268686868687	14.423200889481\\
5.33388888888889	14.9225380597142\\
5.45509090909091	15.3589107685253\\
5.57629292929293	15.7516222334821\\
5.69749494949495	16.1115746248819\\
5.81869696969697	16.4455755960613\\
5.93989898989899	16.7581887687292\\
6.06110101010101	17.0526391755073\\
6.18230303030303	17.3313000782857\\
6.30350505050505	17.5959742032963\\
6.42470707070707	17.8480656746935\\
6.54590909090909	18.0886900355255\\
6.66711111111111	18.3187473249571\\
6.78831313131313	18.5389721212653\\
6.90951515151515	18.7499686660067\\
7.03071717171717	18.9522359907043\\
7.15191919191919	19.1461861274542\\
7.27312121212121	19.3321573825073\\
7.39432323232323	19.5104239667494\\
7.51552525252525	19.6812028350522\\
7.63672727272727	19.8446582891724\\
7.75792929292929	20.000904687912\\
7.87913131313131	20.1500074470817\\
8.00033333333333	20.2919823755624\\
8.12153535353535	20.4267932630347\\
8.24273737373737	20.5543474915235\\
8.36393939393939	20.6744892657095\\
8.48514141414141	20.7869898172006\\
8.60634343434343	20.8915335916159\\
8.72754545454545	20.9876989022604\\
8.84874747474747	21.0749307059524\\
8.96994949494949	21.152501801509\\
9.09115151515152	21.2194564498132\\
9.21235353535354	21.2745263420707\\
9.33355555555556	21.3160012947709\\
9.45475757575758	21.3415222783722\\
9.5759595959596	21.3477335381832\\
9.69716161616162	21.3296608028316\\
9.81836363636364	21.2795081441788\\
9.93956565656566	21.184068589054\\
10.0607676767677	21.01824127292\\
10.1819696969697	20.7244668484279\\
10.3031717171717	20.1103220326091\\
10.4243737373737	17.8224131216505\\
10.5455757575758	20.5132006252157\\
10.6667777777778	21.2818799064725\\
10.7879797979798	21.7856259877391\\
10.9091818181818	22.175358497426\\
11.0303838383838	22.5004097565674\\
11.1515858585859	22.7831736948821\\
11.2727878787879	23.0357251443363\\
11.3939898989899	23.265317697579\\
11.5151919191919	23.4766448669143\\
11.6363939393939	23.6729118434766\\
11.757595959596	23.8563974228871\\
11.878797979798	24.0287717661012\\
12	24.1912869288813\\
};
\end{axis}

\begin{axis}[%
width=7.385in,
height=3.073in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
